Improving Model Alignment Through Collective Intelligence of Open-Source LLMS

Building helpful and harmless large language models (LLMs) requires effective model alignment approach based on human instructions and feedback, which necessitates high-quality human-labeled data. Constructing such datasets is often expensive and hard to scale, and may face potential limitations on diversity and generalization. To address these challenges, we introduce Mixture of Agents Alignment (MoAA), that leverages the collective strengths of various language models to provide high-quality data for model alignment. By employing MoAA, we enhance both supervised fine-tuning and preference optimization, leading to improved performance compared to using a single model alone to generate alignment data (e.g. using GPT-4o alone). Evaluation results show that our approach can improve win rate of LLaMA-3.1-8B-Instruct from 19.5 to 48.3 on Arena-Hard and from 22.33 to 57.23 on AlpacaEval2, highlighting a promising direction for model alignment through this new scalable and diverse synthetic data recipe. Furthermore, we demonstrate that MoAA enables a self-improvement pipeline, where models finetuned on MoA-generated data surpass their own initial capabilities, providing evidence that our approach can push the frontier of open-source LLMs without reliance on stronger external supervision. Data and code will be released.

==> Tables/DPO_MoA_paradigm_ablation.tex <==
\begin{table}[t!]
\centering
\caption{Performance comparison of models using different preference learning methods. \textit{MoA-OnPolicy} uses the SFT model to generate on-policy responses in a MoA style, with the SFT model as the aggregator and unchanged proposers. \textit{MoA-OffPolicy} uses the MoA architecture in stage 1 to generate responses. Both settings generate 5 candidate responses with a temperature of 0.8 and use ArmoRM-Llama3-8B-v0.1 as the reward model.}
\label{tab:MoA-paradigm}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Model}  & \textbf{AlpacaEval2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
Llama-3.1-8B-Instruct-\methodnameAbbr-Stage1 & 43.77 & 8.33 & 40.8 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-MoA-OnPolicy & \textbf{57.35} & 8.26 & 43.8 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-MoA-OffPolicy & 51.59 & 8.44 & 43.2 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-Stage2 & 57.23 & \textbf{8.58} & \textbf{48.3} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/DPO_RM_ablation.tex <==
\begin{table}[t]
\centering
\caption{Performance comparison of models using different reward models. All settings generate five candidate responses with a temperature of 0.8 and use the reward model to pick chosen and rejected responses as the preference pair. We use the same \textit{Llama-3.1-8B-Instruct-SFT} as the base model for DPO across all setups.}
\label{tab:RM-ablation}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Reward Model} & \textbf{AlpacaEval 2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
Llama-3.1-70B-Instruct & 55.35 & 8.36 & 45.1 \\
Qwen2-72B-Instruct & 55.80 & 8.31 & 43.5 \\
Gemma-2-27B-it & 56.81 & 8.31 & \textbf{48.8} \\
{\color{red}GPT-4o-2024-0806} & {\color{red}55.05} & {\color{red}\textbf{8.76}} & {\color{red}44.1} \\
MoA as reward model & \textbf{57.23} & 8.58 & 48.3 \\
  \\
 ArmoRMLlama3-8B-v0.1 & \textbf{57.79} & \textbf{8.56} & \textbf{42.3} \\
  PairRM \citep{llm-blender-2023} & 50.17 & 8.33 & 42.2 \\
  \\
   \textit{N/A (SFT Reference)} & \textit{43.77} & \textit{8.33} & \textit{40.8} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/RewardBench_results.tex <==
\begin{table}[t]
\centering
\small
\caption{Performance comparison of the MoA reward model and other widely-used reward models on Rewardbench.}
\begin{tabular}{llcccc|c}
\toprule
\textbf{Model Type} & \textbf{Method/Model} & \textbf{Chat} & \textbf{Chat Hard} & \textbf{Safety} & \textbf{Reasoning} & \textbf{Average} \\
\midrule
\multirow{3}{*}{Open-Source} 
&Llama-3.1-70B-Instruct & \textbf{97.2} & \textbf{70.2} & 82.8 & 86.0 & 84.0 \\
&Gemma-2-27B-it & 94.8 & 59.1 & 86.4 & 83.3  & 80.9 \\
&Qwen2-72B-Insutrct & 96.2 & 64.6 & 86.0 & 86.1  & 83.2 \\
&MoA as reward model     & 94.7 & 69.4 & \textbf{90.6} & \textbf{87.7} & \textbf{85.6} \\
\\
\multirow{2}{*}{Fine-Tuned} 
&ArmoRM-Llama3-8B-v0.1  & {\color{red}\textbf{96.9}}  & {\color{red}\textbf{76.8}} & {\color{red}\textbf{90.5}} & {\color{red}\textbf{97.3}} & {\color{red}\textbf{90.4}}\\
&PairRM  & 90.2 & 52.2 & 47.7 & 49.0 & 59.8 \\
{\color{red}Closed-Source} & {\color{red}GPT-4o-2024-05-13}  & {\color{red}96.6} & {\color{red}70.4} &  {\color{red}86.5} & {\color{red}84.9} & {\color{red}84.6} \\

\bottomrule
\end{tabular}
\label{tab:rewardbench_results}
\end{table}


==> Tables/SFT_multi_model_ablation.tex <==
\begin{table}[t!]
\centering
\caption{Model performances by SFT on data generated by baseline multi-model methods and MoA. We finetune on Llama-3.1-8B-Instruct with the same training setups as MoA-SFT including the dataset. Combine 5: including all five responses generated by each individual model. Random 5: random sampling of one response from the five models for each instruction. Best of 5: choosing the best response out of five models for each instruction using ArmoRM-Llama3-8B-v0.1.}
\label{tab:SFT-multi-model-ablation}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Method}  & \textbf{AlpacaEval 2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
% Llama-3-8B-Instruct & 22.9 & 8.0 & 20.6 \\
Llama-3.1-8B-Instruct & 22.33 & 8.01 & 19.5 \\
Combined 5 & 27.23 & 8.17 & 26.7 \\
Random 5 & 25.30 & 8.19 & 26.4 \\
Best of 5 & 35.62 & \textbf{8.36} & 38.6 \\
\text{Llama-3.1-8B-Instruct-\methodnameAbbr-SFT} & \textbf{43.77} & {\color{red}8.33} & \textbf{40.8} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/SFT_single_model_ablation.tex <==
\begin{table}[t]
\centering
\caption{
Model performances by SFT on the data generated by single models and MoA. All models are tuned on the original Llama-3.1-8B-Instruct. The \textbf{Teacher} column indicates the model used to generate the data for SFT. We use UF + UC as the dataset for all experiments.
}
\label{tab:SFT-single-model-ablation}
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Model} &\textbf{Teacher} & \textbf{AlpacaEval 2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
% Llama-3-8B-Instruct & 22.9 & 8.0 & 20.6 \\
\multirow{7}{*}{
\makecell[l]{Llama-3.1\\-8B-Instruct}
}

& \textit{N/A (No SFT Reference)} & 22.33 & 8.01 & 19.5 \\
& {\color{red}\textit{N/A (Original Data)}} & {\color{red}14.50} & {\color{red}7.73} & {\color{red}11.7} \\
& Llama-3.1-70B-Instruct & 14.53 & 7.84 & 10.4 \\
& Qwen2-72B-Instruct & 20.50 & 7.88 & 19.5 \\
& Llama-3.1-405B-Instruct & 24.26 & 8.06 & 25.2 \\
&Gemma-2-27B-it & 36.86 & 8.12 & 31.4 \\
&Wizardlm-2-8x22B & 33.26 & 8.44 & 36.5 \\
&GPT-4o-05-13 & 33.95 & \textbf{8.55} & 36.9 \\
& \methodnameAbbr-SFT & \textbf{43.77} & 8.33 & \textbf{40.8} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/criteria_filtering_rewaredBench_results.tex <==
\begin{table}[t]
\centering
\small
\caption{Performance comparison of MoA with and without criteria filtering on Rewardbench. }
\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \textbf{Chat} & \textbf{Chat Hard} & \textbf{Safety} & \textbf{Reasoning} & \textbf{Average} \\
\midrule
MoA without Filtering  & \textbf{95.5}  & 68.8 & 88.1 & 85.6 & 84.5 \\
MoA with Filtering     & 94.7 & \textbf{69.4} & \textbf{90.6} & \textbf{87.7} & \textbf{85.6} \\
\bottomrule
\end{tabular}
\label{tab:filtering_rewardbench_results}
\end{table}


==> Tables/criteria_filtering_tempalte.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Prompt to select evaluation criteria for responses from reward modeling.}
    \begin{tabular}{@{}p{1\linewidth}@{}}
    \toprule
    Analyze the following user query and two AI assistant responses. Your task is to determine the three most relevant evaluation criteria for assessing these responses. Choose exactly 3 criteria from the list below that are most applicable to this specific query and responses:
    \\\\
    1. Instruction adherence: How well the response follows the user's instructions. \\
    2. Relevance: How directly the response addresses the user's query. \\
    3. Accuracy: The correctness and up-to-date nature of the information provided. \\
    4. Depth: The comprehensiveness and level of detail in the answer. \\
    5. Clarity: How well-structured and easy to understand the response is. \\
    6. Helpfulness: How useful the response is in solving the user's problem or answering their question. \\
    7. Safety: How well the response handles potentially sensitive or dangerous requests. \\
    8. Robustness: How well the response handles nuanced or ambiguous aspects of the query. \\
    \\
    Here's an example to guide your selection and output formatting:
    \\
    Example User Query: "What are the health benefits of drinking green tea?" \\
    Example Assistant A Response: "Green tea has many health benefits. It contains antioxidants that can improve brain function and fat loss. It may also lower the risk of certain cancers and cardiovascular diseases." \\
    Example Assistant B Response: "Green tea is good for you. It has stuff that helps your brain and makes you lose weight. It might also stop you from getting sick." \\
    \\
    Example Output: \\
    Selected Criteria: \\
    1. Accuracy \\
    2. Depth \\
    3. Clarity \\
    \\
    Explanation: For this query about health benefits of green tea, accuracy is crucial to ensure the information provided is correct. Depth is important to cover the range of potential benefits comprehensively. Clarity is necessary to ensure the information is presented in an understandable manner, especially when dealing with scientific health information. \\
    \\
    Now, please analyze the following actual query and responses:
    \\
    User query: \{question\} \\
    Assistant A response: \{answer\_a\} \\
    Assistant B response: \{answer\_b\} \\
    \\
    Output your selected criteria strictly using the following format: \\
   Selected Criteria: \\
    1. [Criterion 1] \\
    2. [Criterion 2] \\
    3. [Criterion 3] \\
    \\
    Explanation: [Briefly explain why you chose these three criteria] \\
    \bottomrule
    \end{tabular}
    \label{tab:moj_prompt_criteria_filtering}
\end{table}


==> Tables/data_ablation.tex <==
\begin{table}[t]
\centering
\caption{The influence of instruction tuning set compositions on the model performance. We pick three different sets: Ultrafeedback (UF), Ultrachat (UC), and a mixture of the two (UF + UC). Ultrafeedback has roughly 61,000 data points. Ultrachat we sampled 60,000 data points. And for the mixture, we include all Ultrafeedback data and 5,000 Ultrachat samples.}
\label{tab:data-ablation}
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Model}  & \textbf{MOAA Data}  & \textbf{AlpacaEval 2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
\multirow{3}{*}{Llama-3.1-8B-Instruct} & Ultrafeedback & 39.92 & 8.10 & 39.8 \\
 & Ultrachat & \textbf{43.86} & \textbf{8.39} & 39.5 \\
 & UF + UC & 43.77 & 8.33 & \textbf{40.8} \\
\\
\multirow{3}{*}{{\color{red} Gemma-2-9B-it}} & Ultrafeedback & 51.56 & 7.88 & 45.4 \\
 & Ultrachat & 51.43 & \textbf{8.67} & 45.1 \\
  & UF + UC & \textbf{53.79} & {\color{red}8.65} & \textbf{47.6} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/main_results.tex <==
\begin{table}[t!]
\centering
\caption{Model performances after applying our MoA alignment approach. We demonstrate MoAA-SFT and MoAA-DPO performances for both Llama and Gemma models. \textit{MoA-Data-Generator} row showcases the performance of MoA directly on the benchmarks.}
\label{tab:main-result}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Method}  & \textbf{Size} & \textbf{AlpacaEval 2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
Mistral-7B-instruct-v0.3 &7B& 19.88 & 7.59 & 16.3 \\
Llama-3.1-8B-Instruct & 8B & 22.33 & 8.01 & 19.5 \\
Qwen2.5-7B-Instruct & 7B & 19.91 & 8.22 & 24.6 \\
Gemma-2-9B-it & 9B & 47.43 & 8.48 & 42.0 \\
Gemma-2-27B-it & 27B & \textbf{52.28}  & 8.86 & 54.4 \\
Llama3.1-70B-Instruct & 70B & 37.26  & 8.99 & 55.2 \\
Qwen2-72B-Instruct & 72B & 38.10 & 8.88 & 45.0 \\
{\color{red}Qwen1.5-110B-Instruct} & {\color{red}110B} & {\color{red}43.90} & {\color{red}8.96} & {\color{red}56.4} \\
{\color{red}WizardLM-8x22B} & {\color{red}8x22B} & {\color{red}51.30} & {\color{red}8.78} & {\color{red}\textbf{71.3}} \\
Llama3.1-405b-Instruct & 405B & 40.19  & \textbf{9.18} & 61.5 \\
\\
\text{Llama-3.1-8B-Instruct-\methodnameAbbr-SFT} &8B & \text{43.77} & \text{8.33} & \text{40.8} \\
\text{Llama-3.1-8B-Instruct-\methodnameAbbr-DPO} &8B & \text{57.23} & \text{8.58} & \text{48.3} \\
\text{Gemma-2-9B-it-\methodnameAbbr-SFT} &9B & \text{53.79} & \text{8.65} & \text{47.6} \\
\text{Gemma-2-9B-it-\methodnameAbbr-DPO} &9B & \textbf{63.75} & \textbf{8.91} & \textbf{55.6} \\
\\
\textit{MoA-Data-Generator (Reference)} & - & \textit{62.50} & \textit{9.17} & \textit{75.9} \\

\bottomrule
\end{tabular}
\end{table}

==> Tables/moa_tempalte.tex <==
\begin{table}[h]
    \centering
    \small
    \caption{Aggregate-and-Synthesize Prompt to integrate responses from other models.}
    \begin{tabular}{@{}p{1\linewidth}@{}}
    \toprule
    You have been provided with a set of responses from various open-source models to the latest user query. Your task is to synthesize these responses into a single, high-quality response. It is crucial to critically evaluate the information provided in these responses, recognizing that some of it may be biased or incorrect. Your response should not simply replicate the given answers but should offer a refined, accurate, and comprehensive reply to the instruction. Ensure your response is well-structured, coherent, and adheres to the highest standards of accuracy and reliability.
    \\ \\
    Responses from models:
    \\
    1. [Model Response from $A_{i,1}$] \\
    2. [Model Response from $A_{i,2}$] \\
    ... \\
    $n$. [Model Response from $A_{i,n}$] \\
    \bottomrule
    \end{tabular}
    \label{tab:template}
\end{table}

==> Tables/moj_aggregator_template.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Aggregator prompt for reward modeling.}
    \begin{tabular}{@{}p{1\linewidth}@{}}
    \toprule
    As an expert meta-evaluator, your task is to analyze and synthesize multiple evaluations comparing two AI assistants' responses (A or B) to a user query. Your role is crucial in determining the final assessment. Please consider the following: \\
    \\
    1. Assess the consistency and validity of arguments across all evaluations. \\
    2. Identify any potential biases, errors, or oversights that may have influenced individual evaluations. \\
    3. Consider the strengths and weaknesses of each AI response as highlighted across all evaluations. \\
    4. Synthesize a final, comprehensive evaluation that: \\
    \hspace{5mm} a) Provides a clear comparison of the two AI responses. \\
    \hspace{5mm} b) Addresses any conflicting opinions among the evaluations. \\
    \hspace{5mm} c) Offers a well-reasoned, definitive judgment on which response better addresses the user query. \\
    \hspace{5mm} d) Strictly using "\textbf{[[A]]}" if assistant A is better, or "\textbf{[[B]]}" if assistant B is better to indicate your preferred response. \\
    \\
    Do not let factors such as response length, assistant names, or the order of presentation influence your decision. \\
    \\
    The evaluation should be based on the following criteria: \\
    \{criteria\} \\
    \\
    User query: \{question\} \\
    Assistant A response: \{answer\_a\} \\
    Assistant B response: \{answer\_b\} \\
    \\
    Individual evaluations: \\
    \{proposer\_evaluations\} \\
    \\
    Final Meta-Evaluation: \\
    \bottomrule
    \end{tabular}
    \label{tab:moj_prompt_aggregator}
\end{table}


==> Tables/moj_proposer_template.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Proposer prompt for reward modeling.}
    \begin{tabular}{@{}p{1\linewidth}@{}}
    \toprule
    As an impartial expert evaluator, your task is to critically assess the responses provided by two AI assistants (A and B) to a user query. Follow these steps: \\
    \\
    1. Understand the Query: Carefully analyze the user's question or request to grasp its specific nature and requirements. \\
    \\
    2. Criteria: Focus your evaluation on these three criteria. For each criterion, provide a brief assessment of how well each assistant performed, and then compare them directly. \\
    \{criteria\} \\
    \\
    3. Evaluation: For each selected criterion, provide a qualitative assessment using natural language. Consider using the following phrases: \\
    \hspace{5mm} - Exceptional \\
    \hspace{5mm} - Strong \\
    \hspace{5mm} - Satisfactory \\
    \hspace{5mm} - Needs improvement \\
    \hspace{5mm} - Inadequate \\
    \\
    4. Evaluation Process: \\
    - Provide assessment and brief explanation for each criterion \\
    - Summarize key strengths and weaknesses of each response \\
    - Comparative Analysis: \\
    \hspace{5mm} - Compare the overall performance of both responses \\
    \hspace{5mm} - Explain your reasoning process, referring to specific aspects of each response \\
    \hspace{5mm} - Do not let factors such as response length, assistant names, or the order of presentation influence your decision \\
    \bottomrule
    \end{tabular}
    \label{tab:moj_prompt_proposer}
\end{table}


==> Tables/preference_learning.tex <==
\begin{table}[t!]
\centering
\caption{Performances of models after applying our preference learning method.}
\label{tab:main-result-dpo}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Model}  & \textbf{AlpacaEval2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
Llama-3.1-8B-Instruct & 22.33 & 8.01 & 19.5 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-Stage1 &43.77 & 8.33 & 40.8 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-Stage2 & \textbf{57.23} & \textbf{8.58} & \textbf{48.3} \\
\\
Gemma-2-9b-it & 47.43 & 8.48 & 42.0 \\
Gemma-2-9b-it-\methodnameAbbr-Stage1 & 53.79 & 8.65 & 47.6 \\
Gemma-2-9b-it-\methodnameAbbr-Stage2 & \textbf{63.75} & \textbf{8.91} & \textbf{55.6} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables_ICML/DPO_MoA_paradigm_ablation.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Model}  & \textbf{AlpacaEval2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
Llama-3.1-8B-Instruct-\methodnameAbbr-Stage1 & 43.77 & 8.33 & 40.8 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-MoA-OnPolicy & \textbf{57.35} & 8.26 & 43.8 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-MoA-OffPolicy & 51.59 & 8.44 & 43.2 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-Stage2 & 57.23 & \textbf{8.58} & \textbf{48.3} \\
\bottomrule
\end{tabular}
\caption{Performance comparison of models using different preference learning methods. \textit{MoA-OnPolicy} uses the SFT model to generate on-policy responses in a MoA style, with the SFT model as the aggregator and unchanged proposers. \textit{MoA-OffPolicy} uses the MoA architecture in stage 1 to generate responses. Both settings generate 5 candidate responses with a temperature of 0.8 and use ArmoRM-Llama3-8B-v0.1 as the reward model.}
\label{tab:MoA-paradigm}
\end{table}

==> Tables_ICML/SFT_single_model_ablation.tex <==
\begin{table}[t]
\centering
\small
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Model} &\textbf{Teacher} & \textbf{AlpacaEval 2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
% Llama-3-8B-Instruct & 22.9 & 8.0 & 20.6 \\
\multirow{7}{*}{
\makecell[l]{Llama-3.1\\-8B-Instruct}
}

& \textit{N/A (No SFT)} & 22.33 & 8.01 & 19.5 \\
& \textit{N/A (Original Data)} & 14.50 & 7.73 & 11.7 \\
& Llama-3.1-70B-Instruct & 14.53 & 7.84 & 10.4 \\
& Qwen2-72B-Instruct & 20.50 & 7.88 & 19.5 \\
& Llama-3.1-405B-Instruct & 24.26 & 8.06 & 25.2 \\
&Gemma-2-27B-it & 36.86 & 8.12 & 31.4 \\
&Wizardlm-2-8x22B & 33.26 & 8.44 & 36.5 \\
&GPT-4o-05-13 & 33.95 & \textbf{8.55} & 36.9 \\
& \methodnameAbbr-SFT & \textbf{43.77} & 8.33 & \textbf{40.8} \\
\bottomrule
\end{tabular}
}
\caption{
Model performances by SFT on the data generated by single models and MoA. All models are tuned on the original Llama-3.1-8B-Instruct. The \textbf{Teacher} column indicates the model used to generate the data for SFT. We use UF + UC as the dataset for all experiments. \textit{N/A (Original Data)} means we use the original UF + UC without generating responses with any model.
}
\label{tab:SFT-single-model-ablation}
\end{table}

==> Tables_ICML/preference_learning.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Model}  & \textbf{AlpacaEval2 (LC)} & \textbf{MT-Bench} &  \textbf{Arena-Hard} \\
\midrule
Llama-3.1-8B-Instruct & 22.33 & 8.01 & 19.5 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-Stage1 &43.77 & 8.33 & 40.8 \\
Llama-3.1-8B-Instruct-\methodnameAbbr-Stage2 & \textbf{57.23} & \textbf{8.58} & \textbf{48.3} \\
\\
Gemma-2-9b-it & 47.43 & 8.48 & 42.0 \\
Gemma-2-9b-it-\methodnameAbbr-Stage1 & 53.79 & 8.65 & 47.6 \\
Gemma-2-9b-it-\methodnameAbbr-Stage2 & \textbf{63.75} & \textbf{8.91} & \textbf{55.6} \\
\bottomrule
\end{tabular}
\caption{Performances of models after applying our preference learning method.}
\label{tab:main-result-dpo}
\end{table}
